Four-Quark Hadrons: an Updated Review

The past decade witnessed a remarkable proliferation of exotic charmonium-like resonances discovered at accelerators. In particular, the recently observed charged states are clearly not interpretable as q-qbar mesons. Notwithstanding the considerable advances on the experimental side, conflicting theoretical descriptions do not seem to provide a definitive picture about the nature of the so-called XYZ particles. We present here a comprehensive review about this intriguing topic, discussing both those experimental and theoretical aspects which we consider relevant to make further progress in the field. At this state of progress, XYZ phenomenology speaks in favour of the existence of compact four-quark particles (tetraquarks) and we believe that realizing this instructs us in the quest for a firm theoretical framework.

==> tetra-sym.tex <==
\RequirePackage{xspace}
\usepackage{relsize}
\newcommand{\babar}{\mbox{\slshape B\kern-0.1em{\smaller A}\kern-0.1em
    B\kern-0.1em{\smaller A\kern-0.2em R}}\xspace}
\newcommand{\belle}{Belle\xspace}
\newcommand{\lhcb}{LHCb\xspace}
\newcommand{\bes}{BES~III\xspace}
\newcommand{\cdf}{CDF\xspace}
\newcommand{\cms}{CMS\xspace}
\newcommand{\atlas}{ATLAS\xspace}
\newcommand{\Dzero}{D$\varnothing$\xspace}
\newcommand{\cleoc}{CLEO-$c$\xspace}
\newcommand{\cleo}{CLEO\xspace}
\newcommand{\etal}{\xspace{\it et al.}\xspace}

\newcommand{\sectionname}[1]{Sec.#1\xspace}

\newcommand{\ev}{\ensuremath{\mathrm{\,e\kern -0.1em V}}\xspace}
\newcommand{\kev}{\ensuremath{{\mathrm{\,ke\kern -0.1em V}}}\xspace}
\newcommand{\mev}{\ensuremath{{\mathrm{\,Me\kern -0.1em V}}}\xspace}
\newcommand{\gev}{\ensuremath{{\mathrm{\,Ge\kern -0.1em V}}}\xspace}
\newcommand{\tev}{\ensuremath{{\mathrm{\,Ge\kern -0.1em V}}}\xspace}
\newcommand{\pb}{\ensuremath{{\mathrm{\,pb}}}\xspace}
\newcommand{\nb}{\ensuremath{{\mathrm{\,nb}}}\xspace}
\newcommand{\fm}{\ensuremath{{\mathrm{\,fm}}}\xspace}
\newcommand{\jpsi}{\ensuremath{{J\mskip -3mu/\mskip -2mu\psi\mskip 2mu}}\xspace}
\newcommand{\psiprime}{\ensuremath{\psi(2S)}\xspace}
\newcommand{\stuff}{{\color{red} WRITE STUFF}}
\newcommand{\ie}{{\it i.e.}\xspace}
\newcommand{\eg}{{\it e.g.}\xspace}
\newcommand{\BR}{\ensuremath{\mathcal{B}}\xspace}

\newcommand{\Bz}{\ensuremath{B^0}\xspace}
\newcommand{\xxx}[1]{{\color{red} \bf [#1] }}
\newcommand{\figref}[1]{(\figurename{~\ref{#1}})\xspace}
\newcommand{\spect}[4][]{\ensuremath{\ifthenelse{\equal{#1}{}} {} {#1\,} {}^{#2\!} {#3}_{#4}}}

\def\mes        {\mbox{$m_{\rm ES}$}\xspace}
\def\DeltaE     {\ensuremath{{\rm \Delta}E}\xspace}

\def\D       {\ensuremath{D}\xspace}
%%% do NOT use ensuremath here
\def\Dbar    {\kern 0.2em\bar{\kern -0.2em D}{}\xspace}
\def\Db      {\ensuremath{\Dbar}\xspace}
\def\Dz      {\ensuremath{D^0}\xspace}
\def\Dzb     {\ensuremath{\Dbar^0}\xspace}
\def\DzDzb   {\ensuremath{\Dz {\kern -0.16em \Dzb}}\xspace}
\def\Dp      {\ensuremath{D^+}\xspace}
\def\Dm      {\ensuremath{D^-}\xspace}
\def\Dpm     {\ensuremath{D^\pm}\xspace}
\def\Dmp     {\ensuremath{D^\mp}\xspace}
\def\DpDm    {\ensuremath{\Dp {\kern -0.16em \Dm}}\xspace}
\def\Dstar   {\ensuremath{D^*}\xspace}
\def\Dstarb  {\ensuremath{\Dbar^*}\xspace}
\def\Dstarz  {\ensuremath{D^{*0}}\xspace}
\def\Dstarzb {\ensuremath{\Dbar^{*0}}\xspace}
\def\Dstarp  {\ensuremath{D^{*+}}\xspace}
\def\Dstarm  {\ensuremath{D^{*-}}\xspace}
\def\Dstarpm {\ensuremath{D^{*\pm}}\xspace}
\def\Dstarmp {\ensuremath{D^{*\mp}}\xspace}
\def\Ds      {\ensuremath{D^+_s}\xspace}
\def\Dsb     {\ensuremath{D^-_s}\xspace}
\def\Dss     {\ensuremath{D^{*+}_s}\xspace}
\def\Dmix    {\ensuremath{\Dz-\Dzb}\xspace}
\def\etac     {\ensuremath{\eta_c}\xspace}
\def\Kstar  {\ensuremath{K^{*}}\xspace}
\def\Kp  {\ensuremath{K^{+}}\xspace}
\def\Km  {\ensuremath{K^{-}}\xspace}
\def\Kz  {\ensuremath{K^{0}}\xspace}
\def\kaon  {\ensuremath{K}\xspace}
\def\Bbar    {\kern 0.2em\bar{\kern -0.2em B}{}\xspace}
\def\B       {\ensuremath{B}\xspace}
\def\Bp  {\ensuremath{B^{+}}\xspace}
\def\Bz  {\ensuremath{B^{0}}\xspace}
\def\Bzb     {\ensuremath{\Bbar^0}\xspace}
\def\Bstar   {\ensuremath{\B^*}\xspace}
\def\Bstarb   {\ensuremath{\Bbar^*}\xspace}
\def\Bstarp  {\ensuremath{B^{*+}}\xspace}
\def\Bstarzb {\ensuremath{\Bbar^{*0}}\xspace}
\def\DspDsm     {\ensuremath{D^+_s}\ensuremath{D^-_s}\xspace}
\def\DsspDsm     {\ensuremath{D^{*+}_s}\ensuremath{D^-_s}\xspace}
\def\DsspDssm     {\ensuremath{D^{*+}_s}\ensuremath{D^{*-}_s}\xspace}
\def\DssqpDssqm     {\ensuremath{D^{(*)+}_s}\ensuremath{D^{(*)-}_s}\xspace}
\def\Dsp      {\ensuremath{D^+_s}\xspace}
\def\Dsm      {\ensuremath{D^-_s}\xspace}
\def\Dssp     {\ensuremath{D^{*+}_s}\xspace}
\def\Dssm     {\ensuremath{D^{*-}_s}\xspace}
\def\Dssqp     {\ensuremath{D^{(*)+}_s}\xspace}
\def\Dssqm     {\ensuremath{D^{(*)-}_s}\xspace}
\def\Dssq      {\ensuremath{D^{(*)\pm}_s}\xspace}


\def\KS    {\ensuremath{K^0_{\scriptscriptstyle S}}\xspace} 
\def\Kstarz  {\ensuremath{K^{*0}}\xspace}
\def\ccbar {\ensuremath{c\bar c}\xspace}
\def\bbbar {\ensuremath{b\bar b}\xspace}
\def\Lbar     {\kern 0.2em\overline{\kern -0.2em\Lambda\kern 0.05em}\kern-0.05em{}\xspace}


%%% antonello
\def\be{\begin{equation}}
\def\ee{\end{equation}}
\def\bea{\begin{eqnarray}}
\def\eea{\end{eqnarray}}
\def\dq{\mathbbm{q}}
\def\bpm{\begin{pmatrix}}
\def\epm{\end{pmatrix}}
\def\tr{{\mathrm{Tr}}}

%%% colori tabelle
\definecolor{dgreen}{rgb}{0.0, 0.8, 0.0}
\newcommand{\Xseen}   {\textcolor{dgreen}{\bfseries S}\xspace}
\newcommand{\Xnotseen}{\textcolor{red}{\bfseries NS}\xspace}
\newcommand{\Xnotseennow}{F\xspace}
\newcommand{\Xnotdone}{\textcolor{blue}{\bfseries NP}\xspace}
\newcommand{\Xnofit}  {\textcolor{blue}{\bfseries MF}\xspace}
\newcommand{\Xforbid} {---\xspace}
\newcommand{\Xtoohard}{hard\xspace}
